Flying Objects Detection from a Single Moving Camera

We propose an approach to detect flying objects such as UAVs and aircrafts when they occupy a small portion of the field of view, possibly moving against complex backgrounds, and are filmed by a camera that itself moves. Solving such a difficult problem requires combining both appearance and motion cues. To this end we propose a regression-based approach to motion stabilization of local image patches that allows us to achieve effective classification on spatio-temporal image cubes and outperform state-of-the-art techniques. As the problem is relatively new, we collected two challenging datasets for UAVs and Aircrafts, which can be used as benchmarks for flying objects detection and vision-guided collision avoidance.

==> Makefile <==
# Enter here the name of the document (without .tex extension)
doc = top

PDFLATEX = pdflatex
# type "make" to process latex
# type "make refs" to get proper references to figures and papers
# "make ps" and "make pdf" do what you imagine
# "make clean" removes the *~ files of emacs
# "make hardclean" removes the .dvi .aux .log .blg files and the postscript document

quick: 
	@$(PDFLATEX) $(doc).tex || latex $(doc).tex
	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

ns: 
	@pdflatex -interaction=batchmode $(doc).tex || cat $(doc).log | grep "LaTeX Error:"
#	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

refs: 
	@pdflatex -interaction=batchmode $(doc).tex || latex $(doc).tex
	@bibtex $(doc)
	@pdflatex -interaction=batchmode $(doc).tex
	@pdflatex -interaction=batchmode $(doc).tex
	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

up:
	cvs update

co:	commit
commit:
	cvs commit

ps:     refs
	dvips -o $(doc).ps -t letter $(doc).dvi

pdf:	
	latex -interaction=batchmode $(doc).tex || latex $(doc).tex
	bibtex $(doc)
	latex $(doc).tex
	latex $(doc).tex
	dvips -o $(doc).ps -t letter $(doc).dvi
	ps2pdf $(doc).ps
	acroread $(doc).pdf

clean:
	\rm -f *~ 

hardclean:
	\rm -f $(doc).dvi $(doc).ps $(doc).pdf *~ *.aux *.log *.blg *.bbl


==> fig/coll.tex <==
\begin{table}
\centering
\begin{tabular}{lc}
\toprule
& AveP \comment{& BEP} \vspace{-0.5em}\\
\scriptsize{Detection scenario:} &  \scriptsize{(average precision)} \comment{& \scriptsize{(break-even point)}} \vspace{0.5em} \\
Collision situation & 0.907 \comment{& 86.42} \\
General situation & 0.904 \comment{& 83.88} \\
\bottomrule
\end{tabular}
\mycaption{Comparison of the performances of the detector of the aircrafts on the collision course, with its extension to the general flight situations using our motion compensation algorithm.}
\label{tbl:collision_vs_general}
\end{table}


==> fig/planes.tex <==
\newcommand{\mdsz}{0.60in}
\begin{figure}
\centering
\begin{tabular}{cccc}
\includegraphics[width = \mdsz]{./fig/planes/plane_ex_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \mdsz]{./fig/planes/plane_ex_35.png} & 
  \hspace{-0.3cm}\includegraphics[width = \mdsz]{./fig/planes/plane_ex_57.png} & 
  \hspace{-0.3cm}\includegraphics[width = \mdsz]{./fig/planes/plane_ex_91.png} \\
\includegraphics[width = \mdsz]{./fig/planes/plane_ex_184.png} & 
  \hspace{-0.3cm}\includegraphics[width = \mdsz]{./fig/planes/plane_ex_294.png} & 
  \hspace{-0.3cm}\includegraphics[width = \mdsz]{./fig/planes/plane_ex_300.png} & 
  \hspace{-0.3cm}\includegraphics[width = \mdsz]{./fig/planes/plane_ex_319.png} \\
\end{tabular}
\caption{Sample patches illustrate the variety of types of flying objects, which
  appear in the dataset.}
\label{fig:plane_models}
\end{figure}


==> fig/stabilize.tex <==
\begin{figure*}[ht!]
%  \ra{1}
\centering
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{4}{c}{\bf Uniform background} & \multicolumn{4}{c}{\bf Non-uniform background} & \multicolumn{4}{c}{\bf Very noisy background} \\
\midrule
&&&&\multicolumn{4}{c}{No motion compensation} &&&&\\
\cmidrule(r){5-8} 
\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_0_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_0_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_0_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_0_4.png} &
\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_285_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_285_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_285_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_285_4.png} &
\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_37_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_37_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_37_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/nmc_res_37_4.png} \\
\midrule
&&&&\multicolumn{4}{c}{Lucas-Kanade optical flow} &&&&\\
\cmidrule(r){5-8} 
\includegraphics[width = \dbimsz]{./fig/mc/flow_res_0_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_0_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_0_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_0_4.png} &
\includegraphics[width = \dbimsz]{./fig/mc/flow_res_285_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_285_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_285_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_285_4.png} &
\includegraphics[width = \dbimsz]{./fig/mc/flow_res_37_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_37_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_37_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/flow_res_37_4.png}\\
  \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_0.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_0_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_0_y.png} \\   
  \end{tabular}
    }&
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_285.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_285_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_285_y.png} \\   
  \end{tabular}
  } &
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_37.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_37_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/flow_centers_37_y.png} \\   
  \end{tabular}
  }\\
%\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_0_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_0_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_0_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_0_4.png} &
%\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_285_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_285_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_285_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_285_4.png} &
%\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_37_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_37_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_37_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/flow_bg_37_4.png} \\
    \midrule
&&&&\multicolumn{4}{c}{Our approach} &&&&\\
\cmidrule(r){5-8} 
\includegraphics[width = \dbimsz]{./fig/mc/reg_res_0_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_0_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_0_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_0_4.png} &
\includegraphics[width = \dbimsz]{./fig/mc/reg_res_285_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_285_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_285_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_285_4.png} &
\includegraphics[width = \dbimsz]{./fig/mc/reg_res_37_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_37_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_37_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/reg_res_37_4.png}\\
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_0.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_0_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_0_y.png} \\   
  \end{tabular}
    }&
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_285.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_285_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_285_y.png} \\   
  \end{tabular}
  } &
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_37.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_37_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/mc/reg_centers_37_y.png} \\   
  \end{tabular}
  }\\
%\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_0_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_0_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_0_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_0_4.png} &
%\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_285_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_285_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_285_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_285_4.png} &
%\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_37_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_37_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_37_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/mc/mean_sub/reg_bg_37_4.png} \\
\bottomrule
\multicolumn{4}{c}{(a)} & \multicolumn{4}{c}{(b)} & \multicolumn{4}{c}{(c)} \\
\end{tabular}
\mycaption{Compensation for the mUAV apparent motion  inside the st-cube allows to decrease in-class variation of the data, used  by the machine learning algorithms.  The difficulty of the samples increases from  {\bf left} to {\bf right}.  For each \stcb{},  we also  provide three  graphs:  The blue  dots in  the first  graph indicate the locations of the center  of the drone throughout the \stcb{}, the red cross indicates  the patch center. The  next two graphs plot the  variations of the $x$ and $y$  coordinates of the center of the  drone respectively, compared to the position of the center of the patch.  We can see that our method keeps the drone close to the center even for complicated backgrounds and when the drone is barely recognizable as in the right column. }
\label{fig:stabilize}
\end{figure*}



==> fig/stabilize_pl.tex <==
\begin{figure*}[ht!]
%  \ra{1}
\centering
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{4}{c}{\bf Uniform background} & \multicolumn{4}{c}{\bf Non-uniform background} & \multicolumn{4}{c}{\bf Very noisy background} \\
\midrule
&&&&\multicolumn{4}{c}{No motion compensation} &&&&\\
\cmidrule(r){5-8} 
\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_234_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_234_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_234_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_234_4.png} & 
\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_68_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_68_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_68_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_68_4.png} &
\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_23_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_23_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_23_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/nmc_res_23_4.png} \\
\midrule
&&&&\multicolumn{4}{c}{Lucas-Kanade optical flow} &&&&\\
\cmidrule(r){5-8} 
\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_234_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_234_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_234_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_234_4.png} &
\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_68_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_68_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_68_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_68_4.png} &
\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_23_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_23_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_23_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/flow_res_23_4.png}\\
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
  	\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_234.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_234_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_234_y.png} \\   
  \end{tabular}
    }&
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_68.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_68_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_68_y.png} \\   
  \end{tabular}
  } &
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_23.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_23_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/flow_centers_23_y.png} \\   
  \end{tabular}
  }\\
%\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_234_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_234_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_234_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_234_4.png} &
%\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_68_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_68_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_68_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_68_4.png} &
%\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_23_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_23_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_23_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/flow_bg_23_4.png}\\
  \midrule
&&&&\multicolumn{4}{c}{Our approach} &&&&\\
\cmidrule(r){5-8} 
\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_234_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_234_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_234_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_234_4.png} &
\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_68_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_68_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_68_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_68_4.png} &
\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_23_1.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_23_2.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_23_3.png} & 
  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/reg_res_23_4.png}\\
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_234.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_234_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_234_y.png} \\   
  \end{tabular}
    }&
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_68.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_68_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_68_y.png} \\   
  \end{tabular}
  } &
    \multicolumn{4}{c}{
  \begin{tabular}{ccc}
\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_23.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_23_x.png} & 
  \hspace{-0.3cm}\includegraphics[height = \dbimsz]{./fig/pl_mc/reg_centers_23_y.png} \\   
  \end{tabular}
  }\\
%  \includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_234_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_234_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_234_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_234_4.png} &
%\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_68_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_68_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_68_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_68_4.png} &
%\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_23_1.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_23_2.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_23_3.png} & 
%  \hspace{-0.3cm}\includegraphics[width = \dbimsz]{./fig/pl_mc/mean_sub/reg_bg_23_4.png}\\
\bottomrule
\multicolumn{4}{c}{(a)} & \multicolumn{4}{c}{(b)} & \multicolumn{4}{c}{(c)} \\
\end{tabular}
\mycaption{Compensation  for the  aircraft  motion inside  the  st-cube allows  to decrease  in-class  variation  of  the  data, used  by  the  machine  learning algorithms. The  difficulty of the samples  increases from {\bf left}  to {\bf right}.  For  each \stcb{}, we also  provide three graphs: The  blue dots in the first graph  indicate the locations of the center  of the drone throughout the \stcb{},  the red cross  indicates the patch center.  The next two  graphs plot the variations  of  the  $x$ and  $y$  coordinates  of  the  center of  the  drone respectively, compared to the position of the center of the patch. }
\label{fig:mc_plane}
\end{figure*}


